ReposVul: A Repository-Level High-Quality Vulnerability Dataset

Open-Source Software (OSS) vulnerabilities bring great challenges to the software security and pose potential risks to our society. Enormous efforts have been devoted into automated vulnerability detection, among which deep learning (DL)-based approaches have proven to be the most effective. However, the current labeled data present the following limitations: (1) Tangled Patches: Developers may submit code changes unrelated to vulnerability fixes within patches, leading to tangled patches. (2) Lacking Inter-procedural Vulnerabilities: The existing vulnerability datasets typically contain function-level and file-level vulnerabilities, ignoring the relations between functions, thus rendering the approaches unable to detect the inter-procedural vulnerabilities. (3) Outdated Patches: The existing datasets usually contain outdated patches, which may bias the model during training. To address the above limitations, in this paper, we propose an automated data collection framework and construct the first repository-level high-quality vulnerability dataset named ReposVul. The proposed framework mainly contains three modules: (1) A vulnerability untangling module, aiming at distinguishing vulnerability-fixing related code changes from tangled patches, in which the Large Language Models (LLMs) and static analysis tools are jointly employed. (2) A multi-granularity dependency extraction module, aiming at capturing the inter-procedural call relationships of vulnerabilities, in which we construct multiple-granularity information for each vulnerability patch, including repository-level, file-level, function-level, and line-level. (3) A trace-based filtering module, aiming at filtering the outdated patches, which leverages the file path trace-based filter and commit time trace-based filter to construct an up-to-date dataset.

==> Sections/5.1_distribution_figure.tex <==
% % (a)
% \begin{figure}[h]		
% \label{fig:time_pro}
%  % \setlength{\abovecaptionskip}{-0.001cm}
%   \centering
%     \begin{tikzpicture}[scale=0.593]
%         \begin{axis}[
%           xbar stacked,
%           bar width=11.5pt,
%           height=7.3cm,
%           width=11.5cm,
%           axis y line*= none,
%           axis x line*= none,
%           tickwidth=0pt,
%             ticklabel style={font=\LARGE},
%           % enlarge y limits={abs=0.1},
%           xlabel={ \LARGE \bf Time proportion (\%)},
%           symbolic y coords={ bio-SC-GT, econ-beacxc, Slashdot, loc-gowalla,DBLP,web-Google,as-skitter,zhishi-baidu,ew-2013,Friendster},
%           ytick=data,
%             every axis plot/.append style={line width = 1.6pt},
%             every axis/.append style={line width = 1.6pt},
%           legend style={at={(0.5,-0.21)}, anchor=north,legend columns=-1,draw=none},
%           legend entries={{\huge coreReduce},{\huge buildTree}, {\huge updateIter}},
%           legend image code/.code={
%             \draw [#1] (0cm,-0.263cm) rectangle (0.4cm,0.15cm); },
%         ]
%         \addplot[pattern=north west lines, pattern color=c1] coordinates {(0.58,bio-SC-GT) (0.00,econ-beacxc)(1.4,Slashdot)(6.7,loc-gowalla) (30.7,DBLP) (32.7,web-Google) (0.16,as-skitter) (2.7,zhishi-baidu) (3,ew-2013) (8.3,Friendster)};
%         \addplot[pattern=north east lines , pattern color=c2 ] coordinates {(20.2,bio-SC-GT) (3.06,econ-beacxc)(27.3,Slashdot) (60.2,loc-gowalla) (46.1,DBLP) (39.2,web-Google) (15.55,as-skitter) (32.7,zhishi-baidu) (71.1,ew-2013) (67.1,Friendster)};
%         % \addplot[fill=selectInitCand,pattern=crosshatch, pattern color=c3] 
%         \addplot[pattern=crosshatch, pattern color=c8] coordinates {(79.22,bio-SC-GT) (96.94,econ-beacxc) (71.3,Slashdot)(33.1,loc-gowalla) (23.2,DBLP) (28.1,web-Google) (84.29,as-skitter) (64.6,zhishi-baidu) (25.9,ew-2013) (24.6,Friendster) };
%         \end{axis}
%     \end{tikzpicture}
% \caption{Proportion of time cost of each step in {\Method}.}
% \label{fig:exp:proportion}
% \end{figure}

% % (b)

% \definecolor{c1}{RGB}{255,196,115} % OUR
% \definecolor{c2}{RGB}{178,37,42} % w/o knowledge
% \definecolor{c3}{RGB}{103,150,118} % w/o intent
% \definecolor{c4}{RGB}{181,181,181} % w/o reason

% % nmethod

% \pgfplotstableread[row sep=\\,col sep=&]{
% 	k & BM-25 & SBERT & CodeT5   \\
% 	1 & 0.447 & 0.436 & 0.442  \\
% 	2 & 0.451 & 0.476 & 0.447 \\
% 	3 & 0.453 & 0.500 & 0.464 \\
% 	4 & 0.449 & 0.533 & 0.469 \\
%  	5 & 0.453 & 0.529 & 0.440 \\
%         6 & 0.473 & 0.536 & 0.451 \\
%         7 & 0.473 & 0.578 & 0.427 \\
%         8 & 0.462 & 0.573 & 0.418 \\
%         9 & 0.440 & 0.560 & 0.418 \\
% }\MASR

% \pgfplotstableread[row sep=\\,col sep=&]{
% 	k & BM-25 & SBERT & CodeT5   \\
% 	1 & 0.371 & 0.353 & 0.364  \\
% 	2 & 0.362 & 0.397 & 0.355 \\
% 	3 & 0.373 & 0.425 & 0.374 \\
% 	4 & 0.367 & 0.436 & 0.370 \\
%  	5 & 0.380 & 0.445 & 0.351 \\
%         6 & 0.377 & 0.446 & 0.364 \\
%         7 & 0.384 & 0.487 & 0.350 \\
%         8 & 0.382 & 0.476 & 0.342 \\
%         9 & 0.368 & 0.500 & 0.338 \\
% }\MAMA

% \pgfplotstableread[row sep=\\,col sep=&]{
% 	k & BM-25 & SBERT & CodeT5   \\
% 	1 & 0.520  & 0.551 & 0.520  \\
% 	2 & 0.542 & 0.591 & 0.567 \\
% 	3 & 0.560 & 0.604 & 0.573 \\
% 	4 & 0.564 & 0.649 & 0.578 \\
%  	5 & 0.569 & 0.649 & 0.571 \\
%         6 & 0.596 & 0.667 & 0.587 \\
%         7 & 0.580 & 0.707 & 0.578 \\
%         8 & 0.576 & 0.698 & 0.558 \\
%         9 & 0.576 & 0.716 & 0.580 \\
% }\CASR

% \pgfplotstableread[row sep=\\,col sep=&]{
% 	k & BM-25 & SBERT & CodeT5   \\
% 	1 & 0.477 & 0.501 & 0.474  \\
% 	2 & 0.492 & 0.541 & 0.520 \\
% 	3 & 0.513 & 0.561 & 0.522 \\
% 	4 & 0.517 & 0.585 & 0.521 \\
%  	5 & 0.530 & 0.587 & 0.514 \\
%         6 & 0.535 & 0.602 & 0.532 \\
%         7 & 0.526 & 0.633 & 0.525 \\
%         8 & 0.528 & 0.640 & 0.509 \\
%         9 & 0.530 & 0.644 & 0.524 \\
% }\CAMA

% \begin{figure*}[h]
% %  \setlength{\abovecaptionskip}{-0.1cm}
% %   \setlength{\belowcaptionskip}{-0.5cm}
% %   \setlength{\floatsep}{-5.5cm}
% 	\centering		
%     % \ref{named1} \ref{named2} \ref{named3}\\
% 	\subfigure[Success Rate in method-level]{
% 		\begin{tikzpicture}[scale=0.50]
% 			\begin{axis}[
% 			    legend style = {
% 				    legend columns=3,
% 				    draw=none,
% 				},
% 				% width=0.46\textwidth,
%     % 			height=0.36\textwidth,
% 				% legend to name,
% 				xtick = {1,2,3,4,5,6,7,8,9},
% 				xticklabels = {1,2,3,4,5,6,7,8,9},
% 				ymin=0.40,ymax=0.62,
% 				ytick = {0.45, 0.50, 0.55, 0.60},
% 				mark size=2.5pt, 
% 				ylabel={\large \bf SuccessRate@3},
% 				xlabel={\large \bf Number of examples}, 
% 				% ticklabel style={font=\Huge},
% 				ticklabel style={font=\large},
% 				every axis plot/.append style={line width = 2pt},
% 				every axis/.append style={line width = 1.5pt},
% 				]
% 				\addplot [mark=star,color=c1] table[x=k,y=BM-25]{\MASR};
% 				\addplot [mark=pentagon*,color=c2] table[x=k,y=SBERT]{\MASR};
% 				\addplot [mark=diamond*,color=c3] table[x=k,y=CodeT5]{\MASR};
				
% 				% \addlegendentry{$x$}
% 				\legend{BM-25, SBERT, CodeT5}
% 			\end{axis}
% 		\end{tikzpicture}
% 		\label{fig:res/pre.SHS}
% 	}
% 	%
% 	\subfigure[MAP in method-level]{
% 		\begin{tikzpicture}[scale=0.50]
% 			\begin{axis}[
% 			    legend style = {
% 				    legend columns=3,
% 				    draw=none,
% 				},
% 				% width=0.46\textwidth,
%     % 			height=0.36\textwidth,
% 				% legend to name,
% 				xtick = {1,2,3,4,5,6,7,8,9},
% 				xticklabels = {1,2,3,4,5,6,7,8,9},
% 				ymin=0.30,ymax=0.54,
% 				ytick = {0.35, 0.4, 0.45, 0.50},
% 				mark size=2.5pt, 
% 				ylabel={\large \bf MAP@3},
% 				xlabel={\large \bf Number of examples}, 
% 				% ticklabel style={font=\Huge},
% 				ticklabel style={font=\large},
% 				every axis plot/.append style={line width = 2pt},
% 				every axis/.append style={line width = 1.5pt},
% 				]
% 				\addplot [mark=star,color=c1] table[x=k,y=BM-25]{\MAMA};
% 				\addplot [mark=pentagon*,color=c2] table[x=k,y=SBERT]{\MAMA};
% 				\addplot [mark=diamond*,color=c3] table[x=k,y=CodeT5]{\MAMA};
				
% 				% \addlegendentry{$x$}
% 				\legend{BM-25, SBERT, CodeT5}
% 			\end{axis}
% 		\end{tikzpicture}
% 		\label{fig:res/pre.SHS}
% 	}
% 	%
% 	\subfigure[Success Rate in class-level]{
% 		\begin{tikzpicture}[scale=0.50]
% 			\begin{axis}[
% 			    legend style = {
% 				    legend columns=3,
% 				    draw=none,
% 				},
% 				% width=0.46\textwidth,
%     % 			height=0.36\textwidth,
% 				% legend to name,
% 				xtick = {1,2,3,4,5,6,7,8,9},
% 				xticklabels = {1,2,3,4,5,6,7,8,9},
% 				ymin=0.50,ymax=0.77,
% 				ytick = {0.55, 0.60, 0.65, 0.70},
% 				mark size=2.5pt, 
% 				ylabel={\large \bf SuccessRate@3},
% 				xlabel={\large \bf Number of examples}, 
% 				% ticklabel style={font=\Huge},
% 				ticklabel style={font=\large},
% 				every axis plot/.append style={line width = 2pt},
% 				every axis/.append style={line width = 1.5pt},
% 				]

% 				\addplot [mark=star,color=c1] table[x=k,y=BM-25]{\CASR};
% 				\addplot [mark=pentagon*,color=c2] table[x=k,y=SBERT]{\CASR};
% 				\addplot [mark=diamond*,color=c3] table[x=k,y=CodeT5]{\CASR};
				
% 				% \addlegendentry{$x$}
% 				\legend{BM-25, SBERT, CodeT5}
% 			\end{axis}
% 		\end{tikzpicture}
% 		\label{fig:res/pre.SHS}
% 	}
% 	%
%         \subfigure[MAP in class-level]{
% 		\begin{tikzpicture}[scale=0.50]
% 			\begin{axis}[
% 			    legend style = {
% 				    legend columns=3,
% 				    draw=none,
% 				},
% 				% width=0.46\textwidth,
%     % 			height=0.36\textwidth,
% 				% legend to name,
% 				xtick = {1,2,3,4,5,6,7,8,9},
% 				xticklabels = {1,2,3,4,5,6,7,8,9},
% 				ymin=0.45,ymax=0.69,
% 				ytick = {0.50, 0.55, 0.60, 0.65},
% 				mark size=2.5pt, 
% 				ylabel={\large \bf MAP@3},
% 				xlabel={\large \bf Number of examples}, 
% 				% ticklabel style={font=\Huge},
% 				ticklabel style={font=\large},
% 				every axis plot/.append style={line width = 2pt},
% 				every axis/.append style={line width = 1.5pt},
% 				]
% 				\addplot [mark=star,color=c1] table[x=k,y=BM-25]{\CAMA};
% 				\addplot [mark=pentagon*,color=c2] table[x=k,y=SBERT]{\CAMA};
% 				\addplot [mark=diamond*,color=c3] table[x=k,y=CodeT5]{\CAMA};
				
% 				% \addlegendentry{$x$}
% 				\legend{BM-25, SBERT, CodeT5}
% 			\end{axis}
% 		\end{tikzpicture}
% 		\label{fig:res/pre.SHS}
% 	}
% 	\caption{Experimental results with different examples in method-level recommendation and class-level recommendation.}
% 	\label{fig:para_method}
% % 	\vspace{-0.3cm} 
% \end{figure*}


% \pgfplotstableread[row sep=\\,col sep=&]{
%       datasets  & without & with   \\
%     2 & 0.38  & 0.50    \\ 
%     4 & 0.256 & 0.516   \\
%     6 & 0.431 & 0.502  \\
% }\MSR


% \pgfplotstableread[row sep=\\,col sep=&]{
%       datasets & without & with    \\
%     2 & 0.30 & 0.42    \\
%     4 & 0.203 & 0.45   \\
%     6 & 0.349 & 0.416  \\
% }\MMA


% \pgfplotstableread[row sep=\\,col sep=&]{
%       datasets  & without & with   \\
%     2 & 0.43 & 0.64    \\
%     4 & 0.323 & 0.609   \\
%     6 & 0.549 & 0.642  \\
% }\CSR	

% \pgfplotstableread[row sep=\\,col sep=&]{
%       datasets & without & with    \\
%     2 & 0.38  & 0.59     \\
%     4 & 0.275 & 0.551   \\
%     6 & 0.474 & 0.565  \\
% }\CMA

% \begin{figure*}[h]	

% 	\subfigure[Success Rate in method-level]{
%     	\begin{tikzpicture}[scale=0.50]
%     		\begin{axis}[
%     	    	ybar=0pt,
%     			bar width=0.7cm,
% 				% width=0.35\textwidth,
%     % 			height=0.4\textwidth,
%     			xlabel={\large \bf large language model}, 
%                     xmin=1.0,xmax=7.0,
%                     xtick=data,	xticklabels={\Large GPT3.5,\Large ChatGPT, \Large GPT4.0},
%                 % legend style={in={(0.5,0.98)},
%                 % anchor=north,legend columns=-1,
%                 % draw=none},
%                 legend style = {
% 				    legend columns=-1,
% 				    draw=none,
% 				},
% 				legend image code/.code={
%                     \draw [#1] (0cm,-0.18cm) rectangle (0.8cm,0.08cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.28cm) rectangle (1.2cm,0.2cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.263cm) rectangle (1.2cm,0.085cm); },
%     % 			xmin=0.5,xmax=9.5,
%     			ytick = {0.25, 0.35, 0.45, 0.55},
%     			ymin=0.2,ymax=0.57,
%     			tick align=inside,
% 				% yticklabels = {$10^0$, $10^1$, $10^2$, $10^3$, $10^4$,  INF},
%     			ticklabel style={font=\large},
%    			  every axis plot/.append style={line width = 1.2pt},
%     			every axis/.append style={line width = 1.5pt},
%     			ylabel={\large \textbf{SuccessRate@3}},
%     			]
%     			\addplot[pattern=north west lines, pattern color=c1] table[x=datasets,y=without]{\MSR};
%     			\addplot[pattern = horizontal lines ,pattern color=c2] table[x=datasets,y=with]{\MSR};
%     			% \addplot[pattern = crosshatch,pattern color=c3] table[x=datasets,y=32]{\MSR};
%     			% \addplot[pattern = north east lines,pattern color=c1] table[x=datasets,y=64]{\MSR};
%     			\legend{zero-shot LLM, {\tool}-LLM}
    
%     		\end{axis}
%     	\end{tikzpicture}
%     	\label{fig:res-para-shs}
% 	}
% 	%
% 	\subfigure[MAP in method-level]{
%     	\begin{tikzpicture}[scale=0.50]
%     		\begin{axis}[
%     	    	ybar=0pt,
%     			bar width=0.7cm,
% 				% width=0.35\textwidth,
%     % 			height=0.4\textwidth,
%     			xlabel={\large \bf large language model}, 
%                     xmin=1.0,xmax=7.0,
%                     xtick=data,	xticklabels={\Large GPT3.5,\Large ChatGPT, \Large GPT4.0},
%                 % legend style={in={(0.5,0.98)},
%                 % anchor=north,legend columns=-1,
%                 % draw=none},
%                 legend style = {
% 				    legend columns=-1,
% 				    draw=none,
% 				},
% 				legend image code/.code={
%                     \draw [#1] (0cm,-0.18cm) rectangle (0.8cm,0.08cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.28cm) rectangle (1.2cm,0.2cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.263cm) rectangle (1.2cm,0.085cm); },
%     % 			xmin=0.5,xmax=9.5,
%     			ytick = {0.20, 0.30, 0.40, 0.50},
%     			ymin=0.15,ymax=0.52,
%     			tick align=inside,
% 				% yticklabels = {$10^0$, $10^1$, $10^2$, $10^3$, $10^4$,  INF},
%     			ticklabel style={font=\large},
%    			  every axis plot/.append style={line width = 1.2pt},
%     			every axis/.append style={line width = 1.5pt},
%     			ylabel={\large \textbf{MAP@3}},
%     			]
%     			\addplot[pattern=north west lines, pattern color=c1] table[x=datasets,y=without]{\MMA};
%     			\addplot[pattern = horizontal lines ,pattern color=c2] table[x=datasets,y=with]{\MMA};
%     			% \addplot[pattern = crosshatch,pattern color=c3] table[x=datasets,y=32]{\MSR};
%     			% \addplot[pattern = north east lines,pattern color=c1] table[x=datasets,y=64]{\MSR};
%     			\legend{zero-shot LLM, {\tool}-LLM}
    
%     		\end{axis}
%     	\end{tikzpicture}
%     	\label{fig:res-para-shs}
% 	}
% 	%
% 	\subfigure[Success Rate in class-level]{
%     	\begin{tikzpicture}[scale=0.50]
%     		\begin{axis}[
%     	    	ybar=0pt,
%     			bar width=0.7cm,
% 				% width=0.35\textwidth,
%     % 			height=0.4\textwidth,
%     			xlabel={\large \bf large language model}, 
%                     xmin=1.0,xmax=7.0,
%                     xtick=data,	xticklabels={\Large GPT3.5,\Large ChatGPT, \Large GPT4.0},
%                 % legend style={in={(0.5,0.98)},
%                 % anchor=north,legend columns=-1,
%                 % draw=none},
%                 legend style = {
% 				    legend columns=-1,
% 				    draw=none,
% 				},
% 				legend image code/.code={
%                     \draw [#1] (0cm,-0.18cm) rectangle (0.8cm,0.08cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.28cm) rectangle (1.2cm,0.2cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.263cm) rectangle (1.2cm,0.085cm); },
%     % 			xmin=0.5,xmax=9.5,
%     			ytick = {0.35, 0.45, 0.55, 0.65},
%     			ymin=0.3,ymax=0.7,
%     			tick align=inside,
% 				% yticklabels = {$10^0$, $10^1$, $10^2$, $10^3$, $10^4$,  INF},
%     			ticklabel style={font=\large},
%    			  every axis plot/.append style={line width = 1.2pt},
%     			every axis/.append style={line width = 1.5pt},
%     			ylabel={\large \textbf{SuccessRate@3}},
%     			]
%     			\addplot[pattern=north west lines, pattern color=c1] table[x=datasets,y=without]{\CSR};
%     			\addplot[pattern = horizontal lines ,pattern color=c2] table[x=datasets,y=with]{\CSR};
%     			% \addplot[pattern = crosshatch,pattern color=c3] table[x=datasets,y=32]{\MSR};
%     			% \addplot[pattern = north east lines,pattern color=c1] table[x=datasets,y=64]{\MSR};
%     			\legend{zero-shot LLM, {\tool}-LLM}
    
%     		\end{axis}
%     	\end{tikzpicture}
%     	\label{fig:res-para-shs}
% 	}
% 	%
%         \subfigure[MAP in class-level]{
%     	\begin{tikzpicture}[scale=0.50]
%     		\begin{axis}[
%     	    	ybar=0pt,
%     			bar width=0.7cm,
% 				% width=0.35\textwidth,
%     % 			height=0.4\textwidth,
%     			xlabel={\large \bf large language model}, 
%                     xmin=1.0,xmax=7.0,
%                     xtick=data,	xticklabels={\Large GPT3.5,\Large ChatGPT, \Large GPT4.0},
%                 % legend style={in={(0.5,0.98)},
%                 % anchor=north,legend columns=-1,
%                 % draw=none},
%                 legend style = {
% 				    legend columns=-1,
% 				    draw=none,
% 				},
% 				legend image code/.code={
%                     \draw [#1] (0cm,-0.18cm) rectangle (0.8cm,0.08cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.28cm) rectangle (1.2cm,0.2cm); },
%                 % legend image code/.code={
%                 %     \draw [#1] (0cm,-0.263cm) rectangle (1.2cm,0.085cm); },
%     % 			xmin=0.5,xmax=9.5,
%     			ytick = {0.30, 0.40, 0.50, 0.60},
%     			ymin=0.25,ymax=0.65,
%     			tick align=inside,
% 				% yticklabels = {$10^0$, $10^1$, $10^2$, $10^3$, $10^4$,  INF},
%     			ticklabel style={font=\large},
%    			  every axis plot/.append style={line width = 1.2pt},
%     			every axis/.append style={line width = 1.5pt},
%     			ylabel={\large \textbf{MAP@3}},
%     			]
%     			\addplot[pattern=north west lines, pattern color=c1] table[x=datasets,y=without]{\CMA};
%     			\addplot[pattern = horizontal lines ,pattern color=c2] table[x=datasets,y=with]{\CMA};
%     			% \addplot[pattern = crosshatch,pattern color=c3] table[x=datasets,y=32]{\MSR};
%     			% \addplot[pattern = north east lines,pattern color=c1] table[x=datasets,y=64]{\MSR};
%     			\legend{zero-shot LLM, {\tool}-LLM}
    
%     		\end{axis}
%     	\end{tikzpicture}
%     	\label{fig:res-para-shs}
% 	}
	
%         \caption{Experimental results with different large language models in method-level recommendation and class-level recommendation.}
%         \label{fig:para_llm}

% \end{figure*}


==> other_file/3_workflow_old.tex <==
\subsection{Data collection}


Our initial dataset is acquired through a three-step process: vulnerability entry collection, fix patch collection, and related files collection:

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{Figures/framework.pdf}
    \caption{The architecture of Our framework}
\label{fig:architecture}
\end{figure*}

\subsubsection{Vulnerability Entry Collection:}
To ensure the authenticity and comprehensiveness of the data, we extract vulnerability information primarily from official websites. Presently, a multitude of organizations collect, organize, and disseminate data pertaining to code defects identified during software development. However, owing to CVE~\cite{CVE} lacking essential CWE (Common Weakness Enumeration) information, CVEdetails~\cite{CVEdetails} omitting programming language details, and both SARD~\cite{SARD} and CWE~\cite{CWE} being aggregated solely based on CWE categories, we employ Mend~\cite{Mend} for the compilation of vulnerability entries. Mend provides open-source tools for the detection and remediation of vulnerabilities, preserving detailed information for CVE (Common Vulnerabilities \& Exposures) entries spanning the last two decades. In particular, we utilize the BeautifulSoup package to systematically retrieve vulnerability entries in chronological order. Each vulnerability entry encompasses particulars like CVE-ID, CVE description, publication date, associated CWE-ID,  CVSS (Common Vulnerability Scoring System) score, patch links, and additional information. Additionally, we perform a rudimentary filtering process, retaining vulnerability entries with complete specific information.

\subsubsection{Fix Patch Collection:}
For each vulnerability entry, we further collect patches related to it. GitHub, as the largest code hosting platform and open source community, provides many features such as version control and sharing collaboration. Considering that most of the patch links of the vulnerability entries come from the historical commits of Github, we make a request to the GitHub API by executing the curl command to obtain the commit id, commit information, commit date, and basic information of the files involved in the commit. In addition, there are a large number of vulnerability patches in two major projects, Andorid and Chrome, but due to their independent code submission platforms and security update reporting websites, the patch information is not involved in GitHub. Therefore, we crawl the patches of these two projects separately, with the patch information for the Android project coming from Google Git and the Chrome project coming from the bugs.chromium website.

\subsubsection{Related files collection:}
Considering developers often alter numerous files in a single patch submission, it is imperative to gather comprehensive details about the files affected by the patch. Such detailed information encompasses file names, programming languages, the content of files before and after the submission, and specific modifications applied to the files. Ultimately, we consolidate all the aforementioned information to ensure that each dataset entry provides specific insights into the vulnerability entry, fix patch, and the alterations made to the files impacted by the patch. The attribute names and their meanings in the dataset are outlined in the Table~\ref{tab:dataset_info}.

After the above three steps of crawling and filtering, we have obtained a total of XX patches and corresponding XX file modifications from XX projects since 2010.

% \begin{table*}[htbp]
%     \centering
%     % \setlength{\tabcolsep}{10mm}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{cll}
%         \toprule
%         & \textbf{Features} & \textbf{Description} \\
%         \midrule
%         \multirow{14}{*}{\textbf{Vulnerability Entry Information}} & CVE-ID &  The CVE that the instance belongs to \\
%          & CWE-ID & The CWE that the instance belongs to \\
%          & Language & The programming language of the CVE \\
%          & CVE-Description & The description of the CVE \\
%          & Publish-Date &  The publish date of the CVE\\
%          & CVSS &  The CVSS score of the CVE  \\
%          & AV &  The Attack Vector of the CVE  \\
%          & AC &  The Attack Complexity of the CVE  \\
%          & PR &  The Privileges Required of the CVE  \\
%          & UI &  The User Interaction of the CVE  \\
%          & S &  The Scope of the CVE  \\
%          & C &  The Confidentiality of the CVE  \\
%          & I &  The Integrity of the CVE  \\
%          & A &  The Integrity of the CVE  \\
%         \midrule
%         \multirow{10}{*}{\textbf{Fix Patch Information}} & Commit-ID &  The commit id of this patch\\
%          & Commit-Message &  The commit message of this patch \\ 
%          & Commit-Date &  The commit date of this patch \\ 
%          & URL & The API-URL of this patch  \\ 
%          & Html-URL & The Html-URL of this patch  \\ 
%          & Project & The project this patch belongs to  \\ 
%          & Windows-Before &  The patches before this patch \\ 
%          & Windows-After &  The patches after this patch \\ 
%          & Parents & The parent patch of this patch  \\ 
%          & Outdated &  The tag for whether this patch is outdated \\
%         \midrule
%         \multirow{9}{*}{\textbf{Related Files Information}} & Html-URL & The Html-URL of this file \\ 
%          & File-Language &  The programming language of this file \\ 
%          & File-Name &  The name of this file \\ 
%          & Code &  The content of this file \\ 
%          & Code-Before &  The content of this file before fix \\
%           & Code-Diff &  The difference of this file before and after fix \\
%          & Outdated-File-Modify &  The tag for whether this file is outdated in file dictionary \\ 
%          & Outdated-File-Before &  The tag for whether this file is outdated in time window before \\
%          & Outdated-File-After &  The tag for whether this file is outdated in time window after \\
%         \bottomrule
%         % 添加更多行
%     \end{tabular}
%     \caption{Specific information for each entry in the initial dataset, including vulnerability entry information, remediation patch information, and related file information}
%     \label{tab:dataset_info}
% \end{table*}

\begin{table*}[htbp]
    \centering
    \setlength{\tabcolsep}{10mm}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{ll}
        \toprule
         \textbf{Features} & \textbf{Description} \\
        \midrule
         \multicolumn{2}{c}{\textbf{Vulnerability Entry Information}} \\ \midrule
         CVE-ID &  The CVE that the instance belongs to \\
          CWE-ID & The CWE that the instance belongs to \\
          Language & The programming language of the CVE \\
          CVE-Description & The description of the CVE \\
          Publish-Date &  The publish date of the CVE\\
          CVSS &  The CVSS score of the CVE  \\
          AV &  The Attack Vector of the CVE  \\
          AC &  The Attack Complexity of the CVE  \\
          PR &  The Privileges Required of the CVE  \\
          UI &  The User Interaction of the CVE  \\
          S &  The Scope of the CVE  \\
          C &  The Confidentiality of the CVE  \\
          I &  The Integrity of the CVE  \\
          A &  The Integrity of the CVE  \\
        \midrule
        \multicolumn{2}{c}{\textbf{Fix Patch Information}} \\ \midrule
          Commit-ID & The commit id of this patch\\
          Commit-Message &  The commit message of this patch \\ 
          Commit-Date &  The commit date of this patch \\ 
          URL & The API-URL of this patch  \\ 
          Html-URL & The Html-URL of this patch  \\ 
          Project & The project this patch belongs to  \\ 
          Windows-Before &  The patches before this patch \\ 
          Windows-After &  The patches after this patch \\ 
          Parents & The parent patch of this patch  \\ 
          Outdated &  The tag for whether this patch is outdated \\
        \midrule
        \multicolumn{2}{c}{\textbf{Related Files Information}} \\ \midrule
         Html-URL & The Html-URL of this file \\ 
          File-Language &  The programming language of this file \\ 
          File-Name &  The name of this file \\ 
          Code &  The content of this file \\ 
          Code-Before &  The content of this file before fix \\
           Code-Diff &  The difference of this file before and after fix \\
          Outdated-File-Modify &  The tag for whether this file is outdated in file dictionary \\ 
          Outdated-File-Before &  The tag for whether this file is outdated in time window before \\
          Outdated-File-After &  The tag for whether this file is outdated in time window after \\
        \bottomrule
        % 添加更多行
    \end{tabular}
    \caption{Specific information for each entry in the initial dataset, including vulnerability entry information, remediation patch information, and related file information}
    \label{tab:dataset_info}
\end{table*}

% For Challenge 1 and Challenge 2, we chose patches based on four programming languages, C,C++, Java and Python, as the object of study. Our rationale is that these four languages have the highest percentage of collected vulnerability patches and have more prominent defect problems in real industrial scenarios. For Challenge 3, we initially give outdated patch labels for all vulnerability patches. Our specific approach is as follows:

% Further, we build on the results of Challenge 1 to give more precise obsolete patch labels for patches based on the above four programming languages. Our specific approach is as follows:

\subsection{Identifying tangled patches}

Existing vulnerability datasets usually consider all file changes in a patch as vulnerability fix-related, and thus simply consider the pre-modification files as vulnerable and the post-modification files as non-vulnerable, which will seriously affect the reliability of the dataset labels. Therefore, we go through a muti-agent approach by combining LLM with static code analysis tools to check whether each file modified in a patch is vulnerability-related or vulnerability-independent.

\subsubsection{LLM Analysis:}
LLM possesses extensive professional domain knowledge and a strong ability to comprehend contextual information. For each modified file within a patch, we initially utilize the tree-sitter tool to extract the functions and classes involved in the diff. Subsequently, we use the modifications and their respective contexts as the primary content for the prompt. Based on the CWE (Common Weakness Enumeration) associated with each patch, we further retrieve detailed information about the CWE, including its causes and recommended solutions, and incorporate this information into the prompt. This approach assists LLM in determining whether the modifications in the file align with the CWE's remediation criteria. Additional prompts serve as supplementary information placed appropriately within the prompt. A complete prompt is illustrated in the Figure~\ref{promt}. LLM assumes the role of an expert in code vulnerabilities and patch fixes. It assesses whether the modifications to the files are relevant to vulnerability remediation. The output is then mapped to either 'YES' or 'NO'.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/prompt.pdf}
    \caption{A sample prompt for LLM}
\label{promt}
\end{figure}

Since LLMs learn based on different corpora and have different sizes of parameter counts, we need to first explore the performance of LLMs and select the best overall performing LLM for subsequent work. We manually collected 20 real fixes from the CWE website involving code changes that may or may not be related to vulnerability fixes. We used the Prompt mentioned above as input and the performance of different LLMs is shown in the Table \ref{challenge1_llm}.

\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule
         & Size &  True & False & Accuracy \\ \midrule
      Baichuan2~\cite{Baichuan} & 7b  & 5 & 15 & 25\% \\ \midrule
      ChatGLM~\cite{Chatglm}  & 6b & 13 & 7 & 65\% \\ \midrule
      ChatGPT~\cite{ChatGPT}  & 20b & 9 & 11 & 45\% \\ \midrule
      Llama2-7b~\cite{Llama}  & 7b & 2 & 18 & 10\% \\ \midrule
      Llama2-13b~\cite{Llama}  & 13b & 4 & 16 & 20\% \\ \midrule
      Tongyi~\cite{TongYi}  & - & \cellcolor{gray!70} 17 & \cellcolor{gray!70} 3 & \cellcolor{gray!70} 85\% \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of results for different LLMs}
    \label{challenge1_llm}
\end{table}

Further, to verify the validity of our prompt, we explored the performance differences between different prompt forms. From the Table \ref{challenge1_prompt}, we can see that the information about the CWE description and its resolution measures has a significant impact on the judgement of LLMs. In addition, the code modification context has a boost on the accuracy of the results. To ensure the reliability of the results, all the above experiments are repeated three times and the final results are obtained by voting.

\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
         &  True & False & Accuracy \\ \midrule
      w/o Code Context   & 16 & 4 & 80\% \\ \midrule
      w/o CWE Description  & 11 & 9 & 55\% \\ \midrule
      w/o CWE Solutions  & 14 & 6 & 70\% \\  \midrule
      All   & \cellcolor{gray!70} 17 & 3 & \cellcolor{gray!70} 85\% \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of results for different Prompts}
    \label{challenge1_prompt}
\end{table}

\subsubsection{Static code tool checking:}
We use a variety of static tools to check whether the files involved in a patch were vulnerable before the modification, and to obtain more detailed warnings or errors from the checking information. git, as a version control tool, can effectively output the differences between the files before and after the commit, i.e., the Diff. therefore, we further determine whether the lines where the warnings or errors are located are included in the line changes of the Diff. Due to the differences in the programming languages and checking rules of different static tools, we use a concatenated approach to identify vulnerability-related files: a file is considered to be vulnerability-related as long as any of the static tools detects an error in the Diff.

Combining the above three steps, we found X vulnerability-related files and Y vulnerability-irrelevant files in all modified files.
      
\subsection{Extracting inter-procedural vulnerabilities}

Most of the current mainstream vulnerability datasets are based on function granularity, but individual functions are not necessarily flawed per se, and the lack of contextual information about individual functions poses an obstacle to model training. Therefore for Challenge 2, we classify the granularity of datasets into line-level, function-level, file-level, and cross-file-level.

\begin{algorithm}[!tpb]
    \SetAlgoLined
    \footnotesize
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Ensure}{Ensure}
    \SetKwFunction{Inter-class Distance Prototype}{Inter-class Distance Prototype}
    \SetKwProg{Fn}{Function}{:}{}
    \Input{Source Code: $\mathcal{X}$, Selected Label: $\mathcal{C}$, Threshold: $T_{max}, T_{min}$}
    \Output{Pseudo-positive Label: {$\mathcal{I}^{HN}$}, Pseudo-negative Label: {$\mathcal{I}^{HP}$}}
    \Ensure{$\Theta$ denotes the pre-trained model, $\Omega$ denotes the current model}
    
\caption{Arithmetic of Challenge 2}
\label{algorithm1}
\end{algorithm}

\subsubsection{Cross-file level:}
First we download the repository corresponding to the patch commit and the repository corresponding to the previous commit. For vulnerability-related files, the APIs called and parameters passed in them are important contextual information. Therefore, we use a static tool to search the repository and extract the APIs and parameters involved in the vulnerability-related files and expand them into files.

\subsubsection{File-level:}
In Challenge 1 we obtained vulnerability-related files versus vulnerability-independent files by filtering. Further, for vulnerability related files, we treat them as vulnerable before modification and non-vulnerable after modification; for vulnerability-independent files, we treat them as non-vulnerable before and after modification.

\subsubsection{Function level:}
We use the tree-sitter tool to extract functions, classes, or other structures built in files. By comparing their changes before modification, we treat the function, class, or structure as vulnerable before modification and non-vulnerable after modification for vulnerability-related files, and as non-vulnerable for vulnerability-independent files.

\subsubsection{Line level:}
We conveniently extract the line changes involved in the modification from the diff information and use the line changes as a more precise detection target, which will help the model to locate them more accurately.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.8\textwidth]{Figures/example.png}
%     \caption{The architecture of Challenge2}
%     \label{fig:architecture}
% \end{figure*}

\subsection{Recognizing outdated patches}

Finding outdated patches is important for building high-quality datasets, as patches may have a time lag and introduce new vulnerabilities. For the vulnerability introduction problem, we use the file dictionary approach, while for the patch lag problem, we use the time window approach. Finally, we filter the patch-related files based on their file suffixes to determine the outdated patches.

\subsubsection{File Dictionary:}
For all collected patches, and all files involved in the patches, we first construct a dictionary of the names of the modified files with their commit dates, and keep only the latest commit date corresponding to that file. Then, we iterate through all the files again, and if the file's commit date is earlier than the date of the corresponding entry in the file dictionary, we consider that the original modification of the file is incomplete or introduces new CVEs, and thus it may be an obsolete file.

\subsubsection{Time Window:}
For all the patches, we fetch the patches in the window before and after using the current patch as the origin by means of git log. Further, we determine whether the files modified in the time window overlap with the files modified by this patch. If there is an overlap, we consider that the overlapping files may be outdated.

\subsubsection{File Suffix Filtering:}
Among the multiple files involved in a patch, some of the files are modified in a way that is not related to the functionality of the project, including the description document .md, .rst, the data files .json, .svg, the project change file .ChangeLog, the output file .out, and so on. Files ending in these extensions may have been modified in the history patch, so they need to be filtered.

% \subsubsection{Accurate Discriminations:}
% In Challenge 1, we obtained the labels of each file in the patch, i.e., whether the modification of the file is related to the vulnerability fix or not, through a combination of LLM and static analysis tools. Therefore, in order to get more precise labels of outdated patches, we make more stringent restrictions based on the previous two steps: both the File Dictionary and the Time Window are for files that are truly vulnerability fix related.

Through the above three steps, we find out all the outdated patches. The analysis of the results of the outdated patches will be described in the fourth part of this paper.

% \begin{table*}[htbp]
%     \centering
%     % \setlength{\tabcolsep}{10mm}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{cclc}
%         \toprule
%         & Granularity & \textbf{Features} & \textbf{Description} \\
%         \midrule 
%         \multirow{8}{*}{\textbf{Additional Information on Related Files}} & \multirow{2}{*}{\textbf{Function}} & Functions &  \\
%          &  & Functions-Before &  \\ \cline{2-4}
%          & \multirow{4}{*}{\textbf{File}} & Static &  \\
%          & & LLM-Check &  \\
%          & & Static-Check &  \\
%          & & Target &  \\ \cline{2-4}
%          & \multirow{2}{*}{\textbf{Inter-procedural}} & Inter-procedural-Code &  \\
%          & & Inter-procedural-Code-Before  &  \\
%         \bottomrule
%         % 添加更多行
%     \end{tabular}
%     \caption{Additional information on related files}
%     \label{tab:dataset_info_more}
% \end{table*}


\begin{table*}[htbp]
    \centering
    % \setlength{\tabcolsep}{10mm}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{clc}
        \toprule
         \textbf{Granularity} & \textbf{Features} & \textbf{Description} \\
        \midrule 
         \multirow{2}{*}{\textbf{Function}} & Functions &  \\
           & Functions-Before &  \\ \midrule
          \multirow{4}{*}{\textbf{File}} & Static &  \\
          & LLM-Check &  \\
          & Static-Check &  \\
          & Target &  \\ \midrule
          \multirow{2}{*}{\textbf{Inter-procedural}} & Inter-procedural-Code &  \\
          & Inter-procedural-Code-Before  &  \\
        \bottomrule
        % 添加更多行
    \end{tabular}
    \caption{Additional information on related files}
    \label{tab:dataset_info_more}
\end{table*}
